Pressure gain combustion for gas turbines: Analysis of a fully coupled engine model

The ``Shockless Explosion Combustion" (SEC) concept for gas turbine combustors, introduced in 2014, approximates constant volume combustion (CVC) by harnessing acoustic confinement of autoigniting gas packets. The resulting pressure waves simultaneously transmit combustion energy to a turbine plenum and facilitate the combustor's recharging against an average pressure gain. Challenges in actualizing an SEC-driven gas turbine include i) the creation of charge stratifications for nearly homogeneous autoignition, ii) protecting the turbo components from combustion-induced pressure fluctuations, iii) providing evidence that efficiency gains comparable to those of CVC over deflagrative combustion can be realized, and iv) designing an effective one-way intake valve. This work addresses challenges i)-iii) utilizing computational engine models incorporating a quasi-one-dimensional combustor, zero- and two-dimensional compressor and turbine plena, and quasi-stationary turbo components. Two SEC operational modes are identified which fire at roughly one and two times the combustors' acoustic frequencies. Results for SEC-driven gas turbines with compressor pressure ratios of 6:1 and 20:1 reveal 1.5-fold mean pressure gains across the combustors. Assuming ideally efficient compressors and turbines, efficiency gains over engines with deflagration-based combustors of 30% and 18% are realized, respectively. With absolute values of 52% and 66%, the obtained efficiencies are close to the theoretical Humphrey cycle efficiencies of 54% and 65% for the mentioned pre-compression ratios. Detailed thermodynamic cycle analyses for individual gas parcels suggest that there is room for further efficiency gains through optimized plenum and combustor designs.

==> settings.tex <==
% !TEX root = main_ASME.tex

\RequirePackage{fix-cm}

%
% \usepackage{mathptmx}      % use Times fonts if available on your TeX system
%\usepackage{bm}
\usepackage[squaren]{SIunits}
%\usepackage[latin9]{inputenc}
%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{amsxtra}
%\usepackage{esint}
%\usepackage{cool}
%\usepackage{booktabs}
%\usepackage{url}
%\usepackage{autobreak}
\usepackage[utf8]{inputenc}
%\usepackage{upgreek,bm}
%\usepackage{rotating}
\usepackage{smaller}
\usepackage{verbatim}
%\usepackage{soul}


\newcommand{\turb}{\text{T}}
\newcommand{\verd}{\text{C}}
\newcommand{\nutz}{\text{out}}
\newcommand{\gh}{\text{gh}}

\newcommand{\rotrate}{N}
\let\rr=\rotrate
\newcommand{\Erot}{E_{\textrm{rot}}}
\newcommand{\InertialMoment}{I}
\newcommand{\rrbar}{\overline{\rotrate}}
\newcommand{\rrmax}{\rotrate_{\textrm{max}}}
\newcommand{\rrmin}{\rotrate_{\textrm{min}}}

\newcommand{\AV}{A_{\textrm{V}}}
\newcommand{\ACTP}{A_{\textrm{I}+\frac{1}{2}}}
\newcommand{\AT}{A_{\textrm{T}}}
\newcommand{\AVPC}{A_{\frac{1}{2}}}

\newcommand{\cp}{c_{\textrm{p}}}
\newcommand{\cref}{c_{\textrm{ref}}}
\newcommand{\CT}{C_{\textrm{T}}}
\newcommand{\cv}{c_{\textrm{v}}}

\newcommand{\eps}{\varepsilon}
\newcommand{\etaV}{\eta_{\textrm{V}}}
\newcommand{\etaT}{\eta_{\textrm{T}}}

\newcommand{\half}{\frac{1}{2}}
\newcommand{\hTP}{h_{\textrm{TP}}}

\newcommand{\LC}{L_{\textrm{C}}}

\newcommand{\pin}{p_{\textrm{ghV}}}
\newcommand{\plast}{p_{I}}
\newcommand{\pbar}{\overline{p}}
\newcommand{\pmax}{p_{\textrm{max}}}
\newcommand{\pmin}{p_{\textrm{min}}}
\newcommand{\pone}{p_{1}}
\newcommand{\pout}{p_{\textrm{ghT}}}
\newcommand{\pref}{p_{\textrm{ref}}}
\newcommand{\pTP}{p_{\textrm{TP}}}
\newcommand{\pvar}{{\Delta p}}
\newcommand{\pV}{p_{\textrm{V}}}
\newcommand{\pVsoll}{p_{\textrm{V}}^{\textrm{soll}}}

\newcommand{\PT}{P_{\textrm{T}}}
\newcommand{\PV}{P_{\textrm{V}}}
\newcommand{\PM}{P_{\textrm{M}}}

\newcommand{\Pibar}{\overline{\Pi}}
\newcommand{\DelPi}{\Delta\Pi}

\newcommand{\rhoin}{\rho_{\textrm{ghV}}}
\newcommand{\rholast}{\rho_{I}}
\newcommand{\rhoone}{\rho_{1}}
\newcommand{\rhoout}{\rho_{\textrm{ghT}}}
\newcommand{\rhoref}{\rho_{\textrm{ref}}}
\newcommand{\rhoTP}{\rho_{\textrm{TP}}}
\newcommand{\rhoV}{\rho_{\textrm{V}}}

\newcommand{\rhoeTP}{(\rho e)_{\textrm{TP}}}


\newcommand{\rhouV}{(\rho u)_{\textrm{V}}}
\newcommand{\rhouVPC}{(\rho u)_{\half}}
%\newcommand{\rhouCTP}{(\rho u)_{\textrm{C-TP}}}
\newcommand{\rhouCTP}{(\rho u)_{\textrm{I}+\frac{1}{2}}}
%\newcommand{\rhohuCTP}{(\rho h u)_{\textrm{C-TP}}}
\newcommand{\rhohuCTP}{(\rho h u)_{\textrm{I}+\frac{1}{2}}}
\newcommand{\rhouTPT}{(\rho u)_{\textrm{TP-T}}}
\newcommand{\rhohuTPT}{(\rho h u)_{\textrm{TP-T}}}

\newcommand{\TE}{T_{\textrm{E}}}
\newcommand{\Tin}{T_{\textrm{ghV}}}
\newcommand{\Tlast}{T_{I}}
\newcommand{\Tone}{T_{1}}
\newcommand{\Tout}{T_{\textrm{ghT}}}
\newcommand{\Tref}{T_{\textrm{ref}}}
\newcommand{\Tstar}{T_{*}}
\newcommand{\Tsw}{T_{\textrm{sw}}}
\newcommand{\TTout}{T_{\textrm{T,out}}}
\newcommand{\TTP}{T_{\textrm{TP}}}
\newcommand{\TV}{T_{\textrm{V}}}

\newcommand{\uin}{u_{\textrm{ghV}}}
\newcommand{\ulast}{u_{I}}
\newcommand{\uone}{u_{1}}
\newcommand{\uout}{u_{\textrm{ghT}}}
\newcommand{\uref}{u_{\textrm{ref}}}

\newcommand{\VTP}{V_{\textrm{TP}}}
\newcommand{\VVP}{V_{\textrm{VP}}}

\newcommand{\Yin}{Y_{\textrm{ghV}}}
\newcommand{\Ylast}{Y_{I}}
\newcommand{\Yout}{Y_{\textrm{ghT}}}
\newcommand{\Ystoech}{Y_{\textrm{st}}}

\newcommand{\tign}{t_{\textrm{ign}}}
\newcommand{\tref}{t_{\textrm{ref}}}
\newcommand{\tvalve}{t_{\textrm{vlv}}}

%\newcommand{\Ma}{\text{Ma}}
\newcommand{\Ma}{\mbox{\textit{Ma}}}
%\renewcommand{\Rey}{\text{Re}}
\newcommand\Rey{\mbox{\textit{Re}}}
%\newcommand{\Sc}{\text{Sc}}
\newcommand{\Sc}{\mbox{\textit{Sc}}}

\renewcommand{\Pr}{\mbox{\textit{Pr}}}
%\renewcommand{\Pr}{\text{Pr}}

\newcommand{\eq}[1]{(\ref{#1})}

\newcommand{\dss}{\displaystyle}

\newcommand{\ie}{\emph{i.e.}}

\newcommand{\rfr}[1]{#1_{\text{ref}}}

\newcommand{\tildethree}{\widetilde{3}}

\newcommand{\order}[1]{^{(#1)}}

\newcommand{\littleoh}[1]{o\left(#1\right)}

%----------------------------------------------------------------------------
%---- Farben und Macros zur Textmarkierung ----------------------------------
%----------------------------------------------------------------------------
\usepackage{color}
\definecolor{light}{gray}{0.50}
\definecolor{heavy}{gray}{0.35}
\definecolor{black}{gray}{0.0}
\definecolor{dgreen}{rgb}{0.0,0.7,0}
\definecolor{dred}{rgb}{0.9959,0,0}
\definecolor{green}{rgb}{0.0,0.99599,0.0}
\definecolor{purple}{rgb}{0.6,0.0,0.4}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\dgreen}[1]{\textcolor{dgreen}{#1}}
\newcommand{\purple}[1]{\textcolor{purple}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\black}[1]{\textcolor{black}{#1}}
\newcommand{\grey}[1]{\textcolor{heavy}{#1}}
\newcommand{\lightgrey}[1]{\textcolor{light}{#1}}

%----------------------------------------------------------------------------
%---- Kommentare ------------------------------------------------------------
%----------------------------------------------------------------------------
\usepackage[dvipsnames]{xcolor}
\newcommand{\klein}[1]{\textcolor{blue}{#1}}
\newcommand{\oevi}[1]{\textcolor{ForestGreen}{{#1}}}
\newcounter{kleincommentno}
\setcounter{kleincommentno}{1}
\newcommand{\kleincomment}[1]{{\small\bfseries\textcolor{blue}{ {\small\bfseries${}^{[\arabic{kleincommentno}]}$}}%
\marginpar{\textcolor{blue}{{\small{\bfseries[\arabic{kleincommentno}]}\ \small #1}}\addtocounter{kleincommentno}{1}}}}

\newcommand{\nadolski}[1]{\textcolor{red}{#1}}
\newcounter{nadolskicommentno}
\setcounter{nadolskicommentno}{1}
\newcommand{\nadolskicomment}[1]{{\small\bfseries\textcolor{red}{ {\small\bfseries${}^{[\arabic{nadolskicommentno}]}$}}%
\marginpar{\textcolor{red}{{\small{\bfseries[\arabic{nadolskicommentno}]}\ \small #1}}\addtocounter{nadolskicommentno}{1}}}}

\newcommand{\oevermann}[1]{\textcolor{ForestGreen}{#1}}
\newcounter{oevermanncommentno}
\setcounter{oevermanncommentno}{1}
\newcommand{\oevermanncomment}[1]{{\small\bfseries\textcolor{ForestGreen}{ {\small\bfseries${}^{[\arabic{oevermanncommentno}]}$}}%
\marginpar{\textcolor{ForestGreen}{{\small{\bfseries[\arabic{oevermanncommentno}]}\ \small #1}}\addtocounter{oevermanncommentno}{1}}}}

\newcommand{\zenker}[1]{\textcolor{magenta}{#1}}
\newcounter{zenkercommentno}
\setcounter{zenkercommentno}{1}
\newcommand{\zenkercomment}[1]{{\small\bfseries\textcolor{magenta}{ {\small\bfseries${}^{[\arabic{zenkercommentno}]}$}}%
\marginpar{\textcolor{magenta}{{\small{\bfseries[\arabic{zenkercommentno}]}\ \small #1}}\addtocounter{zenkercommentno}{1}}}}

\newcommand{\oliver}[1]{\textcolor{orange}{#1}}
\newcounter{olivercommentno}
\setcounter{olivercommentno}{1}
\newcommand{\olivercomment}[1]{{\small\bfseries\textcolor{orange}{ {\small\bfseries${}^{[\arabic{olivercommentno}]}$}}%
\marginpar{\textcolor{orange}{{\small{\bfseries[\arabic{olivercommentno}]}\ \small #1}}\addtocounter{olivercommentno}{1}}}}



